Online Information Acquisition: Hiring Multiple Agents

We investigate the mechanism design problem faced by a principal who hires \emph{multiple} agents to gather and report costly information. Then, the principal exploits the information to make an informed decision. We model this problem as a game, where the principal announces a mechanism consisting in action recommendations and a payment function, a.k.a. scoring rule. Then, each agent chooses an effort level and receives partial information about an underlying state of nature based on the effort. Finally, the agents report the information (possibly non-truthfully), the principal takes a decision based on this information, and the agents are paid according to the scoring rule. While previous work focuses on single-agent problems, we consider multi-agents settings. This poses the challenge of coordinating the agents' efforts and aggregating correlated information. Indeed, we show that optimal mechanisms must correlate agents' efforts, which introduces externalities among the agents, and hence complex incentive compatibility constraints and equilibrium selection problems. First, we design a polynomial-time algorithm to find an optimal incentive compatible mechanism. Then, we study an online problem, where the principal repeatedly interacts with a group of unknown agents. We design a no-regret algorithm that provides $\widetilde{\mathcal{O}}(T^{2/3})$ regret with respect to an optimal mechanism, matching the state-of-the-art bound for single-agent settings.

==> src/app_acc.tex <==
\section{Accessory results}
\begin{lemma}\label{le:lemmaaccessorypart}
	Let $\H\subset\Reals$ be a closed, convex subset of $\Reals$ and $\{\G^1,...,\G^n\}$ be a set of partitions of $\H$, where $\G^i=\{G^i_1,...,G_n^i\}$ with $G^i_j$ convex for each $i,j\in [n]$. Let $\P=\{P_1,...,P_m\}$ be a partition of $\H$ such that for $j\in[n]$, $P_j = \cap_{i\in[n]}G^i_{f(i,j)}$ for some $f(i,j)\in [n]$. Then, it holds that $m \leq n^2 - n + 1$. 
\end{lemma} 
%
\begin{proof}
	Let $\P^{(1)}=\G^1$ and $m(1)=n$. Let now $\P^{(k)}=\{P^{(k)}_1,...,P^{(k)}_{m(k)}\}$, for $m(k)\in \Naturals_{>0}$ be a partition of $\H$ such that for each $j\in [m(k)]$, $P_j^{(k)}$ is convex and $P_j^{(k)} = \cap_{i\in [k]} G^i_{f^{(k)}(i, j)}$, with $f^{(k)}(i, j)\in [n]$. In other words, $\P^{(k)}$ is a set of non-empty and disjoint intervals $P_j^{(k)}\subseteq \H$ such that $\cup_{j\in m(k)}P_j^{(k)} = \H$ in which each element $P_j^{(k)}$ is obtained as the intersection of one element from each $\{\G^1,...\G^k\}$. Similarly, define $\P^{(k-1)}=\{P^{(k-1)}_1,...,P^{(k-1)}_{m(k-1)}\}$, for $m(k-1)\in \Naturals_{>0}$ be a partition of $\H$ such that for each $j\in [m(k-1)]$, $P_j^{(k-1)} = \cap_{i\in [k-1]} G^i_{f^{(k-1)}(i, j)}$ for $f^{(k-1)}(i,j)\in[n]$.
	 Notice that, by definition of $\P^{(k-1)}$, in holds that $\forall j\in [m(k)]$, $P_j^{(k)} = G^k_{a} \cap P_b^{(k-1)}$ for some $a\in [n]$, $b\in [m(k-1)]$. Furthermore, it is easy to see that by convexity of every $P^{(k-1)}_j$ and $G^k_j$, $m(k)$ can be at most $n + m(k-1) - 1$. Thus, we can conclude the following chain of inequalities:
	\[
		m \leq m(n) = n + m(n-1) - 1 \leq 2n + m(n-2) - 2 \leq ... \leq  (n-1) n + m(1) - (n-1) = n^2 - n + 1.
	\]
	This concludes the proof.
\end{proof}

\begin{lemma}[Hoeffding's bound]
	Let $x_1,...,x_n$ be i.i.d. such that $a\leq x_i\leq b$ almost surely for all $i\in [n]$. Furthermore, let $\bar x = \frac{1}{n}\sum_{i\in [n]} x_i$. Then, the following holds for all $\delta\in (0,1)$: 
	\[
		\prob\left(|\bar x - \mathbb{E}\left[\bar x\right]|\leq (b-a)\sqrt{\frac{\ln(2/\delta)}{2n}}\right) \geq 1- \delta.
	\]
\end{lemma}

==> src/app_estcost_old.tex <==
\section{More details on costs estimation}\label{sec:app_estcost}
\begin{algorithm}
	\caption{\algocost}\label{alg:estcost_app}
	\begin{algorithmic}
		\REQUIRE $N_2, N_3, \Gamma, \delta$
		\STATE $\mc V = \{\varnothing\}$
		\FOR{$i\in\N$}
		\FOR{$b_i, b_i^\prime\in B_i\times B_i^\prime$}
		\STATE $\gammavec_i\gets \gammavec_i^{b_i}\in\Gamma_i$
		\STATE $\gammavec_i^\prime\gets \gammavec_i^{b_i^\prime}\in\Gamma_i$
		\STATE $\Lambda_i(b_i, b_i^\prime), \chi_i[b_i, b_i^\prime]\gets\textsc{BS}(i, b_i, b_i^\prime, \gammavec_i, \gammavec_i^\prime, N_2, N_3, \mc V, \Lambda_i, \chivec_i, \delta)$
		\ENDFOR
		\ENDFOR
		\RETURN $\left(\Lambda_i\right)_{i\in\N},\,\max_{i,b_i,b_i^\prime} \chi_i[b_i,b_i^\prime]$
	\end{algorithmic}
\end{algorithm}

In this section we exhaustively describe the algorithm for cost estimation. The pseudocode for the main algorithm is presented in Algorithm~\ref{alg:estcost_app}. For each agent $i\in\N$, the algorithm iteratively explores each pair $b_i,b_i^\prime\in B_i$ to obtain an estimate $\Lambda_i(b_i, b_i^\prime)$ of the cost difference $C_i(b_i, b_i^\prime)$ as well as an high confidence bound $\chi_i[b_i, b_i^\prime]$ such that
%
\[
\Lambda_i(b_i, b_i^\prime) - \chi_i[b_i, b_i^\prime] \leq C_i(b_i, b_i^\prime) \leq \Lambda_i(b_i, b_i^\prime) + \chi_i[b_i, b_i^\prime].
\]
%
To this extent, we leverage the knowledge of scoring rules $\Gamma_i$ described in Assumption~\ref{ass:inc} and use them as starting points of a binary search routine that is described below. As input to the Algorithm, we provide the number of rounds $N_2$, $N_3$ that regulate the amount of rounds used by the binary search routine, the scoring rules $\Gamma$ described in Assumtpion~\ref{ass:inc} and the desired confidence level $\delta$. 

\subsection{Binary search}
%
\begin{algorithm}
	\caption{Binary Search (\textsc{BS})}\label{alg:bs}
	\begin{algorithmic}
		\REQUIRE $i, b_i, b_i^\prime, \gammavec_i, \gammavec^\prime_i, N_2, N_3, \mc V, \Lambda_i, \chivec, \delta$
		\IF{$(b_i, b_i^\prime)\in \mc V$}
		\RETURN $\Lambda_i(b_i, b_i^\prime), \chi_i[b_i, b_i^\prime]$
		\ENDIF
		\STATE $\mc V\gets \mc V \cup \{(b_i, b_i^\prime)\}$
		\STATE $\pi[\svec, a] = 1/d\quad\forall \svec\in\Si,\forall a\in\A$
		\STATE \LComment{Search phase}
		\FOR{$t \in [N_2]$}
		\STATE $\bar\gammavec_i\gets \frac{1}{2}\gammavec_i + \frac{1}{2}\gammavec_i^\prime$
		\STATE Commit to $(\bar\gammavec, \pivec)$ and observe $\tilde b_i^t$	
		\IF{$\tilde b_i^t = b_i$}
		\STATE $\gammavec_i \gets \bar\gammavec_i$
		\ELSIF{$\tilde b_i^t = b_i^\prime$}
		\STATE $\gammavec_i^\prime\gets \bar\gammavec_i$
		\ELSE 
		\STATE \LComment{Split phase}
		\STATE $\Lambda_i(b_i, \tilde b_i^t), \chi_i(b_i, \tilde b_i^t)\gets \textsc{BS}(i, b_i, \tilde b_i^t, \gammavec, \bar\gammavec, N_2, N_3, \mc V, \Lambda_i, \chivec_i, \delta)$
		\STATE $\Lambda_i(\tilde b_i^t, b_i^\prime), \chi_i(\tilde b_i^t, b_i^\prime) \gets \textsc{BS}(i,\tilde b_i^t, b_i^\prime, \bar\gammavec, \gammavec^\prime, N_2, N_3, \mc V, \Lambda_i, \chivec_i, \delta)$
		\RETURN $\Lambda_i(b_i, \tilde b_i^t) + \Lambda_i(\tilde b_i^t, b_i^\prime), \chi_i(b_i, \tilde b_i^t) + \chi_i(\tilde b_i^t, b_i^\prime)$
		\ENDIF	
		\ENDFOR
		\STATE \LComment{Payment estimation phase}
		\STATE Commit for $N_3$ rounds to $(\gammavec, \pivec)$ and observe $\gamma[\tilde s_i^t, \theta^t]$ for $t\in [N_3]$
		\STATE Commit for $N_3$ rounds to $(\gammavec^\prime, \pivec)$ and observe $\gamma^\prime[\tilde s_i^t, \theta^t]$ for $t\in [N_3]$
		\STATE $\Lambda_i(b_i, b_i^\prime), \chi_i(b_i, b_i^\prime)\gets$ compute as in \Cref{eq:costestimators}
		\RETURN $\Lambda_i(b_i, b_i^\prime), \chi_i(b_i, b_i^\prime)$
	\end{algorithmic}
\end{algorithm}
%
The pseudocode for $\textsc{BS}$ is presented in Algorithm~\ref{alg:bs}. For clarity, we fix an agent $i\in\N$ and two actions $b_i,b_i^\prime\in B_i$ and describe the execution of the BS algorithm for estimation of cost difference $C_i(b_i,b_i^\prime)$.  Intuitively, the binary search routine between the two actions $b_i,b_i^\prime\in B_i$ is structured in three distinct phases. The first phase is a \emph{search phase} that implements a search over the space of scoring rules to obtain two uncorrelated scoring rules $\gammavec_i$ $\gammavec_i^\prime: S_i\times\Theta\to [0,M]$ with appropriately bounded distance between them such that $\gammavec_i$ incentivizes\footnote{Recall that an uncorrelated scoring rule $\gammavec_i$ incentivizes an action $b_i$ if $b_i^\circ(\gammavec_i)=b_i$.} action $b_i$ and $\gammavec_i^\prime$ incentivizes action $b_i^\prime$. The second phase, \emph{i.e.,} the \emph{payment estimation phase}, estimates the expected payment received by agent $i$ when the principal commits to the two scoring rules $\gammavec_i$ and $\gammavec_i^\prime$ and uses such estimates to recover an high-confidence interval for the cost difference $C_i(b_i, b_i^\prime)$. The third phase is called \emph{split phase} and is needed to manage all those cases in which the scoring rules found during the search phase are not adequate to recover meaningful upper and lower bounds for the cost difference. 

The algorithm takes as input the agent $i$, the actions $b_i,b_i^\prime$, two uncorrelated scoring rules $\gammavec_i,\gammavec^\prime_i: S_i\times \Theta\to [0,M]$ that incentivize action $b_i$ and $b_i^\prime$, respectively, the desired confidence level $\delta$, the estimates $\Lambda_i$, $\chivec$ found so far, and a set $\mc V\subseteq B_i\times B_i$ that contains all the pairs $b_i, b_i^\prime$ for which the cost difference has already been estimated (this latter is needed to avoid estimating twice the same cost difference). To formalize the characteristics of scoring rules $\gammavec_i,\gammavec_i^\prime$, we define the maximum expected payment received by agent $i$ when the principal commits to an uncorrelated scoring rule $\gammavec_i$ and agent $i$ plays action $b_i\in B_i$, using a best-response policy for signal reporting: 
\[
F_i^\circ(\gammavec_i\vert b_i) = \max_{\varphi: S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta]\right\}.
\]
%
Then, if $\gammavec_i$ incentivizes action $b_i$ and $\gammavec_i^\prime$ incentivizes action $b_i^\prime$, by noticing that ${C_i(b_i, b_i^\prime) = - C_i(b_i^\prime, b_i)}$, we get that
%
\begin{subequations}\label{eq:eqcostboundaux}
	\begin{align}
		F_i^\circ(\gammavec_i\vert b_i) - F_i^\circ(\gammavec_i\vert b_i^\prime) &\geq C_i(b_i, b_i^\prime)\label{eq:incb} \\
		F_i^\circ(\gammavec_i^\prime\vert b_i) - F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) &\leq C_i(b_i, b_i^\prime)\label{eq:incbprime}.
	\end{align}
\end{subequations}
%
\Cref{eq:eqcostboundaux} provides a rather natural way of finding upper and lower bounds to $C_i(b_i, b_i^\prime)$. We will leverage this idea to obtain an estimator for $C_i(b_i,b_i^\prime)$. In the following we distinctly analyze each of the three phases of the algorithm.

\paragraph{Search phase.} 
%
The search phase for agent $i$ between two actions $b_i,b_i^\prime\in B_i$ aims at finding two uncorrelated scoring rules $\gammavec_i,\gammavec_i^\prime$ that satisfy Equations~\eqref{eq:incb}~and~\eqref{eq:incbprime}, while also guaranteeing that $||\gammavec_i - \gammavec_i^\prime||_{\infty}\leq \eta$ for some $\eta>0$. To do so, for $N_2$ rounds we interpolate between the two scoring rules and iteratively update them using the feedback received from the online interaction. In particular, let $\mc T_{d,s}^{(i)}(b_i, b_i^\prime)$ be the set of rounds used by the search phase, when we want to estimate the cost difference $C_i(b_i,b_i^\prime)$. Then, at each $t\in\mc T^{(i)}_{d,s}(b_i,b_i^\prime)$, the principal commits to scoring rule $\bar\gammavec_i = \frac{1}{2}\gammavec_i + \frac{1}{2}\gammavec_i^\prime$ and observes the action $\tilde b_i^t = b_i^\circ(\bar\gammavec_i)$ played by agent $i$. If $\tilde b_i^t = b_i$, the scoring rules $\bar\gammavec_i$ incentivizes action $b_i$ and thus, we proceed by updating $\gammavec_i=\bar\gammavec_i$. Similarly, if $\tilde b_i^t = b_i^\prime$, then the scoring rule $\bar\gammavec_i$ incentivizes action $b_i^\prime$ and we update $\gammavec_i^\prime = \bar\gammavec_i$. If, instead $\tilde b_i^t\neq b_i,b_i^\prime$, we enter the so-called \emph{split phase}, which, for clarity, we describe next. If we never enter the split phase, the search phase ends after $N_2$ rounds (\emph{i.e.,} when $|T^{(i)}_{d,s}(b_i,b_i^\prime)| = N_2$). At this point, scoring rules $\gammavec_i$, $\gammavec_i^\prime$ satisfy Equations~\eqref{eq:incb}~and~\eqref{eq:incbprime}, since the feedback received from the environment guarantees that $b_i^\circ(\gammavec_i) = b_i$ and $b_i^\circ(\gammavec_i^\prime) = b_i^\prime$. Furthermore, we can show the following bound on the distance between the two scoring rules. 
\begin{lemma}\label{le:lemmadistbs}
	For any agent $i\in\N$ and actions $b_i,b_i^\prime\in B_i$, assume the search phase is completed without entering into the split phase. Let $\gammavec_i, \gammavec_i^\prime$ be the scoring rules obtained at the end of the search phase. Then the following holds:
	\[
	|| \gammavec_i - \gammavec_i^\prime||_{\infty}\leq \frac{M}{2^{N_2}}.
	\]
\end{lemma}
%
\begin{proof}
	Fix agent $i$ and actions $b_i,b_i^\prime\in B_i$. Let $d^t$ be the distance between scoring rules $\gammavec_i$ and $\gammavec_i^\prime$ at iteration $t\in T^{(i)}_{d,s}(b_i,b_i^\prime)$. With an abuse of notation, we denote as $d^0$ the distance between the two scoring rules at the beginning of the search phase. Trivially, it holds $d^0 \leq M$. Assume without loss of generality that $\tilde b_i^t = b_i^\prime$. Then, we have that
	\begin{equation}\label{eq:eqdistaux}
		d^{t+1} = ||\gammavec_i - \bar\gammavec_i||_\infty = ||\gammavec_i - \frac{1}{2}\gammavec_i - \frac{1}{2}\gammavec_i^\prime||_\infty = \frac{1}{2}||\gammavec_i - \gammavec_i^\prime||_\infty = \frac{1}{2}d^t.
	\end{equation}
	Thus, by recalling that if we do not enter the split phase, then $|T^{(i)}_{d,s}(b_i,b_i^\prime)|=N_2$, we can iteratively apply \Cref{eq:eqdistaux} to bound $d^{N_2}$ and obtain the result. 
\end{proof}

After the completion of the search phase, the algorithm enters into the payment estimation phase, in which we leverage knowledge of the scoring rules $\gammavec_i, \gammavec_i^\prime$ to recover an estimate of $C_i(b_i,b_i^\prime)$.

\paragraph{Payment estimation phase.}
%
The payment estimation phase starts after the completion of the search phase. In this phase we aim at finding estimates of the expected payments $F_i^\circ(\gammavec_i\vert b_i)$ and $F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$ and then use those to obtain an high-confidence bound for $C_i(b_i,b_i^\prime)$, leveraging both the properties of $\gammavec_i$ and $\gammavec_i^\prime$ mentioned above and \Cref{eq:eqcostboundaux}. In particular, notice that when the principal commits to uncorrelated scoring rule $\gammavec_i$, the payment $\gamma_i[\tilde s_i^t, \theta^t]$ is an unbiased estimate of $F_i^\circ(\gammavec_i\vert b_i)$ since: 
\begin{subequations}
	\begin{align*}
		\mathbb{E}[\gamma_i[\tilde s_i^t, \theta^t]] &= \sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b^\circ(\gammavec_i)\right)\gamma_i[\varphi_i^\circ(s_i\vert\gammavec_i), \theta] \\
		&= \max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma_i[\varphi_i^\circ(s_i\vert\gammavec_i), \theta]\right\}\\
		&= F_i^\circ(\gammavec_i\vert b_i).
	\end{align*}
\end{subequations}
%
Similarly, when the principal commits to scoring rule $\gammavec_i^\prime$ it holds that $\mathbb{E}\left[\gamma_i^\prime[\tilde s_i^t, \theta^t]\right]=F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$. Thus, in order to obtain high confidence bounds for the expected payments $F_i^\circ(\gammavec_i\vert b_i)$ and $F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$, we commit to each one of the two scoring rules for $N_3$ rounds and obtain the following estimates,
\[
\hat F_i^\circ(\gammavec_i\vert b_i) = \frac{1}{N_3}\sum_{t\in \mc T^{(i)}_{d,p}(\gammavec_i)}\gamma_i[\tilde s_i^t, \theta^t]\quad\quad \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) = \frac{1}{N_3}\sum_{t\in \mc T^{(i)}_{d,p}(\gammavec_i^\prime)}\gamma_i^\prime[\tilde s_i^t, \theta^t],
\]
where $\mc T^{(i)}_{d,p}(\gammavec_i)$ denotes the set of round in which the principal committed to scoring rule $\gammavec_i$ during the payment estimation phase. Moreover, using standard concentration arguments, we can provide the following high-confidence bounds for the estimated $\hat F_i^\circ$:
\begin{lemma}\label{le:lemmaestpayment}
	For each $\gammavec_i: S_i\times\Theta\to [0,M]$, for each $\delta\in (0,1)$ and for each $K>0$, the following holds: 
	\[
	\prob\left(|\hat F_i^\circ(\gammavec_i\vert b_i) - F_i^\circ(\gammavec_i\vert b_i)|\leq M\sqrt{\frac{\ln (2K/\delta)}{2N_3}}\right)\geq 1-\frac{\delta}{K},
	\]
	where $b_i=b_i^\circ(\gammavec_i)$.
\end{lemma}
%
\begin{proof}
	The result follows directly from Hoeffding's bound, noticing that for all $t\in\mc T^{(i)}_{d,p}(\gammavec_i)$, $0\leq \gamma_i[\tilde s_i^t, \theta^t] \leq M$, for all $t\in \mc T^{(i)}_{d,p}(\gammavec_i^\prime)$, $0\leq\gamma_i^\prime[\tilde s_i^t, \theta^t]\leq M$ and that 
	\[
	\mathbb{E}\left[\hat F_i^\circ(\gammavec_i\vert b_i)\right] = F_i^\circ(\gammavec_i\vert b_i),\quad\quad \mathbb{E}\left[\hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)\right] = F_i^\circ(\gammavec_i^\prime\vert b_i^\prime).
	\]
\end{proof}

Starting from \Cref{eq:eqcostboundaux}, the last elements needed in order to obtain an high-confidence interval for the cost difference $C_i(b_i, b_i^\prime)$ are estimates for the expected payments $F_i^\circ(\gammavec_i\vert b_i^\prime)$ and  $F_i^\circ(\gammavec_i^\prime\vert b_i)$. We observe that, differently than $F_i^\circ(\gammavec_i\vert b_i)$ and  $F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$, it is not possible to estimate $F_i^\circ(\gammavec_i\vert b_i^\prime)$ and  $F_i^\circ(\gammavec_i^\prime\vert b_i)$ directly using the feedback collected from the online interaction, since every time the principal commits to scoring rule $\gammavec_i$, agent $i$ would respond by playing action $b_i$ rather than action $b_i^\prime$ (the same holds for scoring rule $\gammavec^\prime$ and action $b_i$). Nonetheless, it is possible to leverage the bound on the distance between $\gammavec_i$ and $\gammavec_i^\prime$ shown in Lemma~\ref{le:lemmadistbs} to address this issue. Formally, 
\begin{lemma}\label{le:lemmaclosepayment}
	Let $\gammavec_i,\gammavec_i^\prime:S_i\times\Theta\to [0,M]$ be such that $||\gammavec_i - \gammavec_i^\prime||_\infty\leq \eta$. Then, for each $b_i\in B_i$, the following holds
	\[
	|F_i^\circ(\gammavec\vert b_i) - F_i^\circ(\gammavec_i^\prime\vert b_i)| \leq \eta
	\]
\end{lemma}
\begin{proof}
	Fix $b_i\in B_i$. Let $\bar\varphi,\,\bar\varphi^\prime$ be such that
	\begin{align*}
		\bar\varphi&\in arg\max_{\varphi: S_i\to S_i} \left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta]\right\} \\
		\bar\varphi^\prime&\in arg\max_{\varphi: S_i\to S_i} \left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma^\prime_i[\varphi(s_i), \theta]\right\}.
	\end{align*}
	Then, we have that
	\begin{subequations}
		\begin{align*}
			F_i^\circ(\gammavec\vert b_i) &= \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\bar\varphi(s_i), \theta] \\
			&\geq \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\bar\varphi^\prime(s_i), \theta] \\
			& \geq \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma^\prime_i[\bar\varphi^\prime(s_i), \theta] - \eta \\
			&= F_i^\circ(\gammavec^\prime\vert b_i) - \eta,
		\end{align*}
	\end{subequations}
	and, similarly,
	\begin{subequations}
		\begin{align*}
			F_i^\circ(\gammavec^\prime\vert b_i) &= \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma^\prime_i[\bar\varphi^\prime(s_i), \theta] \\
			&\geq \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\bar\varphi(s_i), \theta] \\
			& \geq \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert b_i\right)\gamma_i[\bar\varphi^\prime(s_i), \theta] - \eta \\
			&= F_i^\circ(\gammavec\vert b_i) - \eta.
		\end{align*}
	\end{subequations}
	Combining the two inequalities, we get
	\[
	F_i(\gammavec^\prime\vert b_i) - \eta \leq F_i(\gammavec\vert b_i) \leq F_i(\gammavec^\prime\vert b_i) + \eta,
	\]
	which gives the result.
\end{proof}
%
In the following, for each agent $i\in\N$, we define as $\mc D_i\subseteq B_i\times B_i$ the set that contains all the couples $(b_i, b_i^\prime)$ for which the execution of the binary search reached the cost estimation phase. Furthermore, for each $i\in\N$ and $b_i,b_i^\prime\in\D_i$, let $\gammavec_{i,b_i}$ and $\gammavec_{i,b_i^\prime}$ be the scoring rules found at the end of the search phase, incentivizing actions $b_i$ and $b_i^\prime$, respectively.
To conclude the analysis of the payment estimation phase and to show how to leverage the results of \Cref{le:lemmadistbs}, \Cref{le:lemmaestpayment} and \Cref{le:lemmaclosepayment} to recover upper and lower confidence bounds for the expected payment $C_i(b_i,b_i^\prime)$, we introduce the auxiliary clean event $\bar\E_d$. 
%
\begin{definition}[Auxiliary clean event for cost estimation]
	The clean event $\bar\E_d$ holds if
	\[
	\begin{split}
		|\hat F_i^\circ(\gammavec_{i, b_i}\vert b_i) - F_i^\circ(\gammavec_{i,b_i}\vert b_i)|&\leq M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}} \\
		|\hat F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) - F_i^\circ(\gammavec_{i,b_i^\prime}\vert b_i^\prime)|&\leq M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}}
	\end{split}\quad\quad \forall i\in\N,\,\forall (b_i,b_i^\prime)\in\D_i.
	\]
\end{definition} 
%
\begin{lemma}\label{le:lemmaauxcleancost}
	The clean event $\bar \E_d$ holds with probability at least $1-\frac{\delta}{2}$.
\end{lemma}
%
\begin{proof}
	By \Cref{le:lemmaestpayment}, we have that 
	\[
	\begin{split}
		\prob\left(|\hat F_i^\circ(\gammavec_{i, b_i}\vert b_i) - F_i^\circ(\gammavec_{i,b_i}\vert b_i)|\leq M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}}\right) &\geq 1- \frac{\delta}{2nk^2} \\
		\prob\left(|\hat F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) - F_i^\circ(\gammavec_{i,b_i^\prime}\vert b_i^\prime)|\leq M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}}\right) &\geq 1- \frac{\delta}{2nk^2}
	\end{split}	\quad\quad \forall i\in\N,\,\forall (b_i,b_i^\prime)\in\D_i.
	\]
	The result follows from a union bound, noticing that 
	\[
	\sum_{i\in\N}\sum_{(b_i,b_i^\prime)\in\D_i} \frac{\delta}{2nk^2} \leq \frac{\delta}{2}.
	\]
\end{proof}
The introduction of the auxiliary clean event allows us to define, for all $i\in\N$ and for all pairs of actions $(b_i, b_i^\prime)\in \D_i$ for which the binary search algorithms reached the cost estimation phase, the following estimators and confidence bounds: 
\begin{subequations}\label{eq:costestimators}
	\begin{align}
		\Lambda_i(b_i, b_i^\prime) &= \hat F_i^\circ(\gammavec_{i, b_i}\vert b_i) - \hat F_i^\circ(\gammavec_{i,b_i^\prime}\vert b_i^\prime), \\
		\chi_i[b_i, b_i^\prime] &= 2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}} + \frac{M}{2^{N_2}}.
	\end{align}
\end{subequations}

We formally prove that, if event $\bar\E_d$ holds, then the above definitions yield, indeed, a valid high-confidence region for the pairwise cost differences. 
\begin{lemma}\label{le:lemmacostsafterpay}
	Assume clean event $\bar\E_d$ holds. Then the following holds:  
	\[
	|\Lambda_i(b_i, b_i^\prime) - C_i(b_i, b_i^\prime)| \leq \chi_i[b_i, b_i^\prime]\quad\quad\forall i\in\N,\,\forall (b_i, b_i^\prime)\in\D_i.
	\]
\end{lemma}
%
\begin{proof}
	Fix $i\in\N$ and $(b_i,b_i^\prime)\in\D$. By \Cref{eq:incb}, we have that
	\begin{subequations}
		\begin{align}
			C_i(b_i, b_i^\prime) &\leq F_i^\circ(\gammavec_{i, b_i}\vert b_i) - F_i^\circ(\gammavec_{i, b_i}\vert b_i^\prime) \\
			&\leq F_i^\circ(\gammavec_{i, b_i}\vert b_i) - F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) + \frac{M}{2^{N_2}} \\
			&\leq \hat F_i^\circ(\gammavec_{i, b_i}\vert b_i) - \hat F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) + \frac{M}{2^{N_2}} + 2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}}, 
		\end{align}
	\end{subequations}
	where the first equation follows from \Cref{le:lemmaclosepayment} and \Cref{le:lemmadistbs}, while the last equation follows from the definition of $\bar\E_d$. Similarly, from \Cref{eq:incbprime}, we get 
	\begin{subequations}
		\begin{align}
			C_i(b_i, b_i^\prime) &\geq F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i) - F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) \\
			&\geq F_i^\circ(\gammavec_{i, b_i}\vert b_i) - F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) - \frac{M}{2^{N_2}} \\
			&\geq \hat F_i^\circ(\gammavec_{i, b_i}\vert b_i) - \hat F_i^\circ(\gammavec_{i, b_i^\prime}\vert b_i^\prime) - \frac{M}{2^{N_2}} - 2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}}, 
		\end{align}
	\end{subequations}
	where, also in this case, the first equation follows from \Cref{le:lemmaclosepayment} and \Cref{le:lemmadistbs}, while the last equation follows from the definition of $\bar\E_d$. The result follows by substituting the definitions of $\Lambda_i(b_i, b_i^\prime)$ and $\chi_i[b_i,b_i^\prime]$.
\end{proof}
%
%
%obtain the following upper and lower bounds for $F_i^\circ(\gammavec_i\vert b_i)$, $F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$, $F_i^\circ(\gammavec_i\vert b_i^\prime)$ and
%it is possible to obtain the following high confidence bounds for the expected payments, 
%\begin{align*}
%	\hat F_i^\circ(\gammavec_i\vert b_i) - M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} &\leq F_i^\circ(\gammavec_i\vert b_i) \leq \hat F_i^\circ(\gammavec_i\vert b_i) + M\sqrt{\frac{\ln (/\delta)}{2N_3}} \\
%	\hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) - M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} &\leq F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) \leq \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) + M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} \\
%	\hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) - M\sqrt{\frac{\ln (2K/\delta)}{2N_3}}- \frac{M}{2^{N_2}} &\leq F_i^\circ(\gammavec_i\vert b_i^\prime) \leq \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) + M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} + \frac{M}{2^{N_2}}\\
%	\hat F_i^\circ(\gammavec_i\vert b_i) - M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} - \frac{M}{2^{N_2}} &\leq F_i^\circ(\gammavec_i^\prime\vert b_i) \leq \hat F_i^\circ(\gammavec_i\vert b_i) + M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} + \frac{M}{2^{N_2}},
%\end{align*}
%where the first two equations follow from Lemma~\ref{le:lemmaestpayment} and the last two equations follow from Lemma~\ref{le:lemmaestpayment} and Lemma~\ref{le:lemmaclosepayment}. Combining the above equations with Equations~\eqref{eq:incb}~and~\eqref{eq:incbprime}, we get:
%%
%\begin{align*}
%		C_i(b_i, b_i^\prime) &\leq \hat F_i^\circ(\gammavec_i\vert b_i) - \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) + 2M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} + \frac{M}{2^{N_2}} \\
%		C_i(b_i, b_i^\prime) &\geq \hat F_i^\circ(\gammavec_i\vert b_i) - \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) - 2M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} - \frac{M}{2^{N_2}}.
%\end{align*}
%
%
%Thus, after the payment estimation phase, the estimator $\Lambda_i(b_i, b_i^\prime)$ and the confidence bounds $\chi_i[b_i, b_i^\prime]$ are 
%\begin{subequations}\label{eq:costestimators}
%	\begin{align}
	%		\Lambda_i(b_i, b_i^\prime) &= \hat F_i^\circ(\gammavec_i\vert b_i) - \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime) \\
	%		\chi_i[b_i, b_i^\prime] &= 2M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} + \frac{M}{2^{N_2}}.
	%	\end{align}
%\end{subequations}
%%
%To conclude the analysis of the payment estimation phase and to show how to leverage \Cref{le:lemmaestpayment} and \Cref{le:lemmaclosepayment} to recover upper and lower confidence bounds for the expected payment $C_i(b_i,b_i^\prime)$, we introduce the auxiliary clean event $\bar\E_d$. 
%%
%\begin{definition}[Auxiliary clean event for cost estimation]
%	For each agent $i\in\N$, Let $\mc D_i\subseteq B_i\times B_i$ be the set that contains all the couples $(b_i, b_i^\prime)$ for which the execution of the binary search reached the cost estimation phase. Furthermore, let $K=2nk^2$. Then, the clean event $\bar\E_d$ holds if	
%	\[
%		|\Lambda_i(b_i, b_i^\prime) - C_i(b_i, b_i^\prime)| \leq \chi_i[b_i, b_i^\prime]\quad\quad\forall i\in\N,\,\forall (b_i, b_i^\prime)\in\D_i,
%	\]
%	where $\Lambda_i(b_i, b_i^\prime) = \hat F_i^\circ(\gammavec_i\vert b_i) - \hat F_i^\circ(\gammavec_i^\prime\vert b_i^\prime)$ and $\chi_i[b_i, b_i^\prime] = 2M\sqrt{\frac{\ln (2K/\delta)}{2N_3}} + \frac{M}{2^{N_2}}$.
%\end{definition} 
%%
%\begin{lemma}\label{le:lemmaauxcleancost}
%	The clean event $\bar\E_d$ holds with probability at least $1-\frac{\delta}{2}$.
%\end{lemma}
%\begin{proof}
%	Fix $i\in\N$ and $b_i, b_i^\prime\in \D_i$. Starting from \Cref{eq:incb} we have that
%	\begin{subequations}
	%		\begin{align}
		%			C_i()
		%		\end{align}
	%	\end{subequations}
%	Notice that by combining Lemma~\ref{le:lemmaestpayment}, Lemma~\ref{le:lemmaclosepayment} and Equation~\eqref{eq:eqcostboundaux} we get that: 
%	\[
%		\prob\left(|\Lambda_i(b_i, b_i^\prime) - C_i(b_i, b_i^\prime)| \leq \chi_i[b_i, b_i^\prime]\right)\geq 1-\frac{\delta}{K}\quad\quad\forall i\in\N,\,\forall (b_i, b_i^\prime)\in\D_i.
%	\]
%	The result follows by a union bound, noticing that 
%	\[
%		\sum_{i\in\N}\sum_{(b_i, b_i^\prime)\in\D_i}\frac{\delta}{2nk^2} \leq \frac{\delta}{2}.
%	\]
%\end{proof}

\paragraph{Split phase.} The analysis of the payment estimation phase suggested that whenever we are able to successfully complete the search phase, then we can easily recover high-confidence regions for the cost differences. However, unfortunately, this is not always the case, since it might happen that during the search phase for an agent $i$ and between two actions $b_i,b_i^\prime\in B_i$, the agent responds with an action $\tilde b_i^t$ which is different than $b_i$ and $b_i^\prime$, thus causing the search phase to end. In such a case, the algorithm enters the split phase. The intuition upon which the design of the split phase is based is that the cost difference $C_i(b_i, b_i^\prime)$ can be expressed in terms of the cost differences $C_i(b_i, \tilde b_i^t)$ and $C_i(\tilde b_i^t, b_i^\prime)$ as follows:
\[
C_i(b_i, b_i^\prime) = C_i(b_i, \tilde b_i^t) + C_i(\tilde b_i^t, b_i^\prime).
\]
Then, this shows that it is possible to recursively obtain an high-confidence interval for $C_i(b_i, b_i^\prime)$ starting from high-confidence intervals for $C_i(b_i, \tilde b_i^t)$ and $C_i(\tilde b_i^t, b_i^\prime)$. In particular, 
\[
\Lambda_i(b_i, \tilde b_i^t) + \Lambda_i(\tilde b_i^t, b_i^\prime) - \chi_i[b_i, \tilde b_i^t] - \chi_i[\tilde b_i^t, b_i^\prime]   \leq C_i(b_i, b_i^\prime) \leq \Lambda_i(b_i, \tilde b_i^t) + \Lambda_i(\tilde b_i^t, b_i^\prime) + \chi_i[b_i, \tilde b_i^t] + \chi_i[\tilde b_i^t, b_i^\prime],
\]
which allows us to define the estimator and confidence bound for $C_i(b_i, b_i^\prime)$ as 
\begin{align*}
	\Lambda_i(b_i, b_i^\prime) &= \Lambda_i(b_i, \tilde b_i^t) + \Lambda_i(\tilde b_i^t, b_i^\prime)\\
	\chi_i[b_i, b_i^\prime] &= \chi_i[b_i, \tilde b_i^t] + \chi_i[\tilde b_i^t, b_i^\prime].
\end{align*}
%
Hence, when the algorithm enters into the split phase, it instantiates two distinct bynary search routines, one for estimating the cost difference $C_i(b_i, \tilde b_i^t)$ using as starting points the scoring rules $\gammavec_i$ and $\bar\gammavec_i$ and the other for estimating $C_i(\tilde b_i^t, b_i^\prime)$ starting from scoring rules $\bar\gammavec_i$ and $\gammavec_i^\prime$. 

We proceed by bounding the number of times the algorithm enters the split phase, thus allowing us to bound the number of rounds used by $\algocost$, as well as the high-confidence bound $\chi = \max_{i,b_i,b_i^\prime}\chi_i[b_i,b_i^\prime]$. To address this question, we consider the binary search procedures instantiated by the main loop of the algorithm. For the sake of presentation, let us fix an agent $i$ and two actions $b_i,b_i^\prime\in B_i$ and consider a binary search between the uncorrelated scoring rules $\gammavec_i^{b}, \gammavec_i^{b^\prime_i}\in\Gamma_i$. Then, the maximum number of times the algorithm enters the split phase during the process of estimating the cost difference $C_i(b_i,b_i^\prime)$ can be characterized by investigating all the possible convex combinations of the two scoring rules $\gammavec_i^{b}, \gammavec_i^{b^\prime_i}$. In particular, we study $\mc H_i(b_i, b_i^\prime) \defeq \hull(\{\gammavec_i^{b}, \gammavec_i^{b^\prime_i}\})$ and introduce \emph{best-response (BR) regions}, \emph{i.e.,} subsets of  $\H_i(b_i, b_i^\prime)$ in which agent $i$'s best response does not change. Since the split phase is entered a number of times that is at most the number of different BR regions, it suffices to bound to number of such regions to recover a bound on the number of rounds used by $\algocost$. Formally, a BR region in which agent $i$'s best response is to play action $\tilde b_i\in B_i$ and to report signals according to policy $\varphi: S_i\to S_i$ is defined as 
\[
\G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) \defeq \left\{\gammavec_i\in \H_i(b_i, b_i^\prime)\mid b_i^\circ(\gammavec_i) = \tilde b_i,\,\varphi_i^\circ(s_i\vert\gammavec_i) = \varphi(s_i)\quad\forall s_i\in S_i\right\}.
\]
%
Trivially, $\H_i(b_i, b_i^\prime) = \cup_{\tilde b_i, \varphi} \G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$. In principle, $\H_i(b_i, b_i^\prime)$ can be partitioned in many BR regions (since the number of different signal reporting policies $\varphi:S_i\to S_i$ is $l^l$). As we show next, there exist in fact a limited number of non-empty BR regions. 
\begin{lemma}\label{le:lemmabrregions}
	For any agent $i$ and actions $b_i,b_i^\prime\in B_i$, there exist at most $k l^2$ non-empty BR regions, \emph{i.e.,} 
	\[
	\left|\left\{(\tilde b_i, \varphi)\mid \G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) \neq \varnothing \right\}\right| \leq k l^2.
	\]
	Furthermore, for each $\tilde b_i\in B_i$ and $\varphi: S_i\to S_i$, the set $\G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$ is convex.
\end{lemma}
%
\begin{proof}
	Fix an agent $i$ and two actions $b_i,b_i^\prime\in B_i$. We first prove the convexity of the BR regions and then we proceed to bound their number.
	
	\paragraph{Convexity.} To prove that the sets $\G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$ are convex for each $\tilde b_i\in B_i$ and $\varphi: S_i\to S_i$, let us explicit the constraints defining such sets. In particular, imposing that $\tilde b_i$ and $\varphi$ are a BR for agent $i$ is equivalent to imposing the following set of constraints:
	%
	\[
	\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\left[\prob^{(i)}\left(s_i, \theta\vert \tilde b_i\right)\gamma_i[\varphi(s_i), \theta] - \prob^{(i)}\left(s_i, \theta\vert \tilde b_i^\prime\right)\gamma_i[\varphi^\prime(s_i), \theta]\right]\geq 0\quad\forall \tilde b_i^\prime\in B_i,\,\forall\varphi^\prime: S_i\to S_i.
	\]
	Clearly, all constraints are linear in $\gammavec_i$, thus implying convexity of the set. 
	
	\paragraph{Bound on the number of non-empty BR regions.} To bound the number of non-empty BR regions, we introduce, for two signals $s_i,s_i^\prime\in S_i$ and an action $\tilde b_i\in B_i$, the set $G_i(\tilde b_i, s_i, s_i^\prime\vert b_i,b_i^\prime)$, containing all those scoring rules $\gammavec_i\in \H_i(b_i, b_i^\prime)$ for which it is a best-response for agent $i$ to report signal $s_i^\prime$ after having played action $\tilde b_i$ and having observed signal $s_i$. Formally, 
	\[
	G_i(\tilde b_i, s_i, s_i^\prime\vert b_i,b_i^\prime) \defeq \left\{\gammavec_i\in\H_i(b_i, b_i^\prime)\mid 	\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert\tilde b_i\right)\left[\gamma_i[s_i^\prime, \theta] - \gamma_i[\tilde s_i, \theta]\right]\geq 0\quad\forall\tilde s_i\in S_i \right\}.
	\]
	Trivially, it holds that $\H_i(b_i, b_i^\prime) = \cup_{s_i^\prime\in S_i} G_i(\tilde b_i, s_i, s_i^\prime\vert b_i,b_i^\prime)$ for all $\tilde b_i\in B_i$ and for all $s_i\in S_i$. 
	%
	Furthermore, for each $\tilde b_i\in B_i$ and $\varphi: S_i\to S_i$, we let with a slight abuse of notation $G_i(\tilde b_i, \varphi\vert b_i,b_i^\prime)$ be the set of scoring rules in $\H_i(b_i, b_i^\prime)$ such that, after having selected action $\tilde b_i$, the best-response policy for agent $i$ is to report signals according to $\varphi$. Formally, 
	\[
	G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) \defeq \left\{\gammavec_i\in H_i(b_i, b_i^\prime)\mid \sum_{\theta\in\Theta}\prob^{(i)}\left(s_i,\theta\vert\tilde b_i\right)\left[\gamma_i[\varphi(s_i), \theta] - \gamma_i[\tilde s_i^\prime, \theta]\right]\geq 0\,\,\forall s_i,s_i^\prime\in S_i\right\}.
	\]
	%
	By definition, each $G_i(\tilde b_i, \varphi \vert b_i, b_i^\prime)$ can be obtained as the intersection of suitably chosen BR regions $G_i(\tilde b_i, s_i, s_i^\prime\vert b_i, b_i^\prime)$, \emph{i.e.,}
	\[
	G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) = \Bigcap_{s_i\in S_i} G_i(\tilde b_i, s_i, \varphi(s_i)\vert b_i, b_i^\prime)\quad\quad\forall \tilde b_i\in B_i,\,\forall \varphi:S_i\to S_i.
	\]
	%
	Furthermore, notice that, since for each $s_i\in S_i$, each set $\{G_i(\tilde b_i, s_i, s_i^\prime\vert b_i, b_i^\prime)\mid s_i^\prime\in S_i\}$ provides a $l$-dimensional partition of $\H_i(b_i, b_i^\prime)$, and since $G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$ is a partition of $\H_i(b_i, b_i^\prime)$, by \Cref{le:lemmaaccessorypart} we can conclude that $|G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)|\leq l^2 - l + 1$. Notice that, in general it holds that for each $\tilde b_i\in B_i$ and $\varphi:S_i\to S_i$, $G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)\supseteq \G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$, since by definition of $G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$, for each $\gammavec_i$ belonging to the set, the signal reporting policy $\varphi$ is a best-response for agent $i$ to $\gammavec_i$ after the agent played action $\tilde b_i$, but nothing guarantees that action $\tilde b_i$ is a best-response itself. To conclude the proof it is enough to notice that, in the worst case, for each $\tilde b_i\in B_i$ and $\varphi: S_i\to S_i$, $G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) = \G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$ and since the number of non-empty $G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime)$ is at most $l^2 - l + 1$, we can conclude that 
	\[
	\left|\left\{(\tilde b_i, \varphi)\mid \G_i(\tilde b_i, \varphi\vert b_i, b_i^\prime) \neq \varnothing \right\}\right| \leq k(l^2 - l + 1) \leq k l^2.
	\] 
	This concludes the proof.
\end{proof}

\Cref{le:lemmabrregions} has another important implication. Since for each $b_i, b_i^\prime\in B_i$, $\H_i(b_i, b_i^\prime)$ can be partitioned in at most $kl^2$ BR regions, the agent will change her action at most $\lfloor \frac{kl^2}{2}\rfloor $ times during the routine for the estimation of $C_i(b_i, b_i^\prime)$, triggering the beginning of a new search phase at most $kl^2$ times. This observation allows us to bound the maximum possible confidence bound as follows 
%
\begin{lemma}\label{le:lemmamaconfcost}
	At the end of the execution of $\algocost$ it holds that 
	\[
	\max_{i\in\N}\max_{b_i, b_i^\prime\in B_i}\chi_i[b_i, b_i^\prime] = 2kl^2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}} + \frac{kl^2M}{2^{N_2}}.
	\]
\end{lemma}
%
\begin{proof}
	For each $i\in\N$ and $b_i, b_i^\prime\in B_i$, let $\D_i(b_i, b_i^\prime)$ be the set that contains all the pairs of actions $(\hat b_i, \hat b_i^\prime)$ for which the payment estimation phase has been reached during the procedure for estimating $C_i(b_i, b_i^\prime)$. Notice that, by \Cref{le:lemmabrregions} it holds that $|\D_i(b_i, b_i^\prime)| \leq kl^2$. Then, by definition of the $\textsc{BS}$ algorithm it follows that 
	\[
	\chi_i[b_i, b_i^\prime] = \sum_{(\hat b_i, \hat b_i^\prime)\in \D_i(b_i, b_i^\prime)} 2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}} + \frac{2M}{2^{N_2}} \leq 2kl^2M\sqrt{\frac{\ln (4nk^2/\delta)}{2N_3}} + \frac{kl^2M}{2^{N_2}}.
	\]
	This concludes the proof.
\end{proof}


\subsection{Formal Guarantees of \algocost}
We conclude this Section by formally proving main properties of Algorithm \ref{alg:estcost_app}. 

\lemmacleancost*
\begin{proof}
	Assume auxiliary clean event $\bar\E_d$ holds. By \Cref{le:lemmacostsafterpay}, for all $i\in\N$ and for all $(b_i, b_i^\prime)\in \D_i$, 
	\[
	|\Lambda_i(b_i, b_i^\prime) - C_i(b_i, b_i^\prime)| \leq \chi_i[b_i, b_i^\prime] \leq \chi.
	\]
	%
	Then, let us fix $i\in\N$ and consider a couple $(b_i, b_i^\prime)\notin \D_i$. Let $\D_i(b_i, b_i^\prime)$ be the set that contains all the pairs of actions $(\hat b_i, \hat b_i^\prime)$ for which the payment estimation phase has been reached during the procedure for estimating $C_i(b_i, b_i^\prime)$. Then, the algorithm guarantees that
	\[
	C_i(b_i, b_i^\prime) = \sum_{(\hat b_i, \hat b_i^\prime)\in\D_i(b_i, b_i^\prime)}C_i(\hat b_i, \hat b_i^\prime).
	\]
	The result follows from \Cref{le:lemmacostsafterpay} noticing that $\D_i(b_i, b_i^\prime)\subset \D_i$.
\end{proof}

\lemmaroundcosts*
\begin{proof}
	Notice that, thanks to the use of the global variable $\mc V$, the payment estimation phase is executed at most $nk^2$ times. Moreover, for each pair $(b_i, b_i^\prime)\in B_i\times B_i$, Lemma~\ref{le:lemmabrregions} guarantees that the split phase is entered at most $kl^2$ times. Thus, the maximum number of rounds devoted to the execution of \algocost\, is at most 
	\[
	|\mc T_d| \leq 2nk^3l^2 N_2 + nk^2N_3.
	\]
\end{proof}
%Algorithm \ref{alg:estcost_app} describes the pseudocode for \algocost. The algorithm, for each agent $i\in\N$, iteratively explores each pair $b_i, b_i^\prime\in B_i$ and exploits a binary search routine in order to estimate the cost difference $C_i(b_i, b_i^\prime)$. The psudocode for $\textsc{BS}$ is provided in Algorithm \ref{alg:bs}. When using binary search to estimate the cost difference $C_i(b_i, b_i^\prime)$ we leverage the knowledge of the uncorrelated scoring rules $\gammavec_i^{b_i}, \gammavec_i^{b_i^\prime}\in\Gamma_i$ described in Assumption \ref{ass:inc} and iteratively interpolate between the two in order to find upper and lower bounds to $C_i(b_i, b_i^\prime)$. More in detail, at each iteration, the algorithm knows an uncorrelated scoring rule $\gammavec_i$ incentivizing action $b_i$ to agent $i$ and a scoring rule $\gammavec_i^\prime$ incentivizing action $b_i^\prime$ to $i$. Then, the principal commits to a mechanism using scoring rule $\bar\gammavec_i = \frac{1}{2}\gammavec_i + \frac{1}{2}\gammavec_i^\prime$ for agent $i$ and observes the action $\tilde b_i^t$ selected by $i$ (\emph{i.e.,} her best response to $\bar\gammavec_i$). If $\tilde b_i^t = b_i$ or $\tilde b_i^t = b_i^\prime$, the procedure continues by updating $\gammavec_i = \bar\gammavec_i$ or $\gammavec^\prime_i = \bar\gammavec_i$, respectively.  Otherwise, if the agent played an action $\tilde b_i^t\neq b_i,b_i^\prime$, then two new \textsc{BS} routines are instantiated in order to estimate the cost differences $C_i(b_i, \tilde b_i^t)$ and $C_i(\tilde b_i^t, b_i^\prime)$, starting from scoring rules $\gammavec_i, \bar\gammavec_i$ and $\bar\gammavec_i, \gammavec_i^\prime$, respectively. Note that, in this latter case, the cost difference $C_i(b_i, b_i^\prime)$ can be written as $C_i(b_i, b_i^\prime) = C_i(b_i, \tilde b_i^t) + C_i(\tilde b_i^t, b_i^\prime)$, and if $|C_i(b_i, \tilde b_i^t) - \Lambda_i(b_i, \tilde b_i^t)|\leq\chi_i[b_i, \tilde b_i^t]$ and $|C_i(\tilde b_i^t, b_i^\prime) - \Lambda_i(\tilde b_i^t, b_i^\prime)|\leq \chi_i[\tilde b_i^t, b_i^\prime]$, then by simple calculations, setting $\Lambda_i(b_i, b_i^\prime) = \Lambda_i(b_i, \tilde b_i^t) + \Lambda_i(\tilde b_i^t, b_i^\prime)$, we obtain
%\[
%|C_i(b_i, b_i^\prime) - \Lambda_i(b_i, b_i^\prime) | \leq \chi_i[b_i, \tilde b_i^t] + \chi_i[\tilde b_i^t, b_i^\prime] = \chi_i[b_i, b_i^\prime], 
%\]
%thus providing an easy way to recover upper and lower bounds for $C_i(b_i, b_i^\prime)$, starting from upper and lower bounds for $C_i(b_i, \tilde b_i^t)$ and $C_i(\tilde b_i^t, b_i^\prime)$. Therefore, if at any $t\in [N_2]$, $\tilde b_i^t\notin\{b_i, b_i^\prime\}$, then the algorithm terminates returning $\Lambda_i(b_i, b_i^\prime)$ and $\chi_i[b_i, b_iì\prime]$ as specified above. Otherwise, if $\tilde b_i^t\in \{b_i, b_i^\prime\}$ for all $t\in [N_2]$, then we have two scoring rules $\gammavec_i$ and $\gammavec^\prime_i$ such that $||\gammavec_i - \gammavec_i^\prime ||_{\infty}\leq M/2^{N_2}$ and
%\begin{subequations}
%	\begin{align*}
	%		&\max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i\\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta] \right\} - \max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i\\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i[\varphi(s_i), \theta] \right\} \geq C_i(b_i, b_i^\prime), \\
	%		&\max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i\\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\} - \max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i\\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\} \leq C_i(b_i, b_i^\prime).
	%	\end{align*}
%\end{subequations}
%%
%To recover meaningful upper and lower bounds for $C_i(b_i, b_i^\prime)$, we observe that when committing to pay agent $i$ according to scoring rule $\gammavec_i$, then the payment $\gamma_i[\tilde s_i^t, \theta^t]$ is an unbiased estimate of $\max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta] \right\}$. Similarly, when committing to scoring rule $\gammavec^\prime_i$, the payment $\gamma_i^\prime[\tilde s_i^t, \theta^t]$ is an unbiased estimate of $\max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\}$. Thus, to estimate both the above expected payments, the principal commits for $N_3$ rounds to scoring rule $\gammavec_i$ and for additional $N_3$ rounds to scoring rule $\gammavec_i^\prime$. Formally, let $\mc T(\gammavec_i)$ and $\mc T(\gammavec_i^\prime)$ be the set of rounds in which the principal used, for agent $i$, scoring rule $\gammavec$ and $\gammavec_i^\prime$, respectively (notice that, by definition, $|\mc T(\gammavec_i)|=|\mc T(\gammavec_i^\prime)|=N_3$). Let us define the following estimators:
%\[
%	\hat F_i(\gammavec_i) = \frac{1}{N_3}\sum_{t\in \mc T(\gammavec_i)} \gamma_i[\tilde s_i^t, \theta^t], \quad\quad\quad
%	\hat F_i(\gammavec_i^\prime) = \frac{1}{N_3}\sum_{t\in \mc T(\gammavec_i^\prime)} \gamma_i[\tilde s_i^t, \theta^t],
%\]
%with $\mathbb{E}[F_i(\gammavec_i)] = \max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta] \right\}$, and $\mathbb{E}[F_i(\gammavec^\prime_i)] = \max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\}$. Simple concentration arguments show that for any $J>0$,  
%\begin{align}
%	\prob\left(\left|\hat F_i(\gammavec_i) - \max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i \\ \theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma_i[\varphi(s_i), \theta] \right\}\right| \leq \sqrt{\frac{M^2\ln(2J/\delta)}{2N_3}}\right) &\geq 1-\frac{\delta}{J}, \label{eq:eq_boundpay1}\\
%	\prob\left(\left|\hat F_i(\gammavec_i^\prime) - \max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i\\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\}\right| \leq \sqrt{\frac{M^2\ln(2J/\delta)}{2N_3}}\right) &\geq 1-\frac{\delta}{J}\label{eq:eq_boundpay2}.
%\end{align}
%
%Unfortunately, it is not possible to directly estimate $\max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i[\varphi(s_i), \theta] \right\}$ and $\max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i\right)\gamma^\prime_i[\varphi(s_i), \theta] \right\}$ by directly interacting with agent $i$, since scoring rules $\gammavec_i$ and $\gammavec_i^\prime$ incentivize, respectively, action $b_i$ over $b_i^\prime$ and action $b_i^\prime$ over $b_i$. However, notice that, since $||\gammavec_i - \gammavec_i^\prime||_\infty \leq M/2^{N_2}$, it is possible to show the following.
%%
%\begin{lemma}\label{le:lemmaauxcost}
%	Let $\gammavec_i, \gammavec_i^\prime: S_i\times\Theta\to[0,M]$ such that $||\gammavec_i - \gammavec_i^\prime||_{\infty}\leq M/2^{N_2}$. Then, for all $b_i, b_i^\prime\in B_i$, the following holds:
%	\[
%		\max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i \\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i[\varphi(s_i), \theta] \right\} - \max_{\varphi:S_i\to S_i}\left\{\sum_{\substack{s_i\in S_i \\\theta\in\Theta}}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i^\prime[\varphi(s_i), \theta]  \right\} \leq \frac{M}{2^{N_2}}.
%	\]
%\end{lemma}
%%
%\begin{proof}
%	To prove the result, let us notice that
%	\begin{subequations}
	%		\begin{align}
		%			&\max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i[\varphi(s_i), \theta] \right\}\notag\\ 
		%			&= \max_{\etavec: S_i\to\Delta (S_i)}\left\{\sum_{s_i\in S_i}\sum_{s_i^\prime\in S_i}\eta[s_i, s_i^\prime]\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i[s_i^\prime, \theta]\right\} \\
		%			&\leq \max_{\etavec: S_i\to\Delta (S_i)}\left\{\sum_{s_i\in S_i}\sum_{s_i^\prime\in S_i}\eta[s_i, s_i^\prime]\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i^\prime[s_i^\prime, \theta]\right\} + \frac{M}{2^{N_2}} \\
		%			&= \max_{\varphi:S_i\to S_i}\left\{\sum_{s_i\in S_i}\sum_{\theta\in\Theta}\prob^{(i)}\left(s_i, \theta\vert b_i^\prime\right)\gamma_i^\prime[\varphi(s_i), \theta]  \right\} + \frac{M}{2^{N_2}}.
		%		\end{align}
	%	\end{subequations}
%	This concludes the proof.
%\end{proof}
%
%Using the result of Lemma \ref{le:lemmaauxcost}, together with Equations \eqref{eq:eq_boundpay1} and \eqref{eq:eq_boundpay2}, we can conclude the following: 
%\[
%	\hat F_i(\gammavec_i) - \hat F_i(\gammavec_i^\prime) - \frac{M}{2^{N_2}} - 2\sqrt{\frac{M^2\ln(2J/\delta)}{2N_3}} \leq C_i(b_i,b_i^\prime) \leq \hat F_i(\gammavec_i) - \hat F_i(\gammavec_i^\prime) + \frac{M}{2^{N_2}} + 2\sqrt{\frac{M^2\ln(2J/\delta)}{2N_3}},
%\]
%which gives: 
%\begin{subequations}
%	\begin{align}
	%		\Lambda_i(b_i, b_i^\prime) &= \hat F_i(\gammavec_i) - \hat F_i(\gammavec_i^\prime)\\
	%		\chi_i[b_i, b_i^\prime] &= \frac{M}{2^{N_2}} + 2\sqrt{\frac{M^2\ln(2J/\delta)}{2N_3}}.
	%	\end{align}
%\end{subequations}

==> src/offline.tex <==
\section{Offline Optimization Problem}\label{sec:offline}
%
Before investigating the online learning problem, we initiate our study by focusing on the offline optimization problem. In particular, we first individuate conditions on the joint probability distribution $\prob\left(\svec, \theta\vert\bvec\right)$ that, if satisfied, guarantee that an uncorrelated mechanism is sufficient to achieve optimal utility for the principal. Next, we show that if the aforementioned conditions are not satisfied, then the introduction of correlated mechanisms allows the principal to achieve higher utility, thus establishing the optimality of correlated mechanisms with respect to uncorrelated mechanisms. Finally, we conclude this section by providing a linear program (LP) formulation for the optimal mechanism which is solvable in polynomial time. 

\subsection{Games with Peer-Independent Signals: Optimality of Uncorrelated Mechanisms}
%
A game with Peer-Independent Signals (PIS game) \fe{Inventare un nome più carino per questi giochi} is a game in which the signals received  by each agent are not affected by the actions performed by the other agents. In this class of games, the state of nature is drawn according to a \emph{prior} probability distribution $\pvec\in\Delta(\Theta)$, while the probability of agent $i$ receiving a signal $s\in S_i$ depends exclusively on the action $b\in B_i$ performed by $i$ and on the state of nature $\theta$, according to a \emph{signaling scheme} $\psi_i(\cdot\vert b, \theta)\in \Delta(S_i)$. Thus, in PIS games, the joint probability distribution $\prob\left(\svec, \theta\vert\bvec\right)$ is given by:
\begin{equation}\label{eq:uncorrprob}
	\prob\left(\svec, \theta\vert\bvec\right) = p[\theta]\prod_{i\in\mc N} \psi_i\left(s_i\vert b_i, \theta \right) \quad \forall \svec\in\Si,\,\forall \theta\in\Theta,\,\forall\bvec\in\B.
\end{equation}

PIS games can model different scenarios related to information acquisition in real-world settings. The following example provides a potential application of this class of games. 
%
\begin{example}[PIS Games]
	Consider the scenario in which a company (the principal) needs to decide whether or not to buy a specific product but they do not have any information on that. In particular, the product can have or not some manufacturing defects (the state of nature) according to some probability distribution (the prior). Furthermore, consider the case in which there are $n$ other companies (the agents) and each of them can conduct different costly experiments (the actions $B_i$) on the product and report, possibly lying, the outcome of the experiments (the signals $S_i$) to the principal. If the principal and the agents can stipulate contracts regulating the amount that the principal will pay to each agent based on the information that the agents reported to the principal and on whether or not the product has actually a manufacturing defect, then this problem can be naturally modeled as a PIS game.
\end{example}

Given the particular information structure of PIS games, as the next theorem shows, there always exists an optimal uncorrelated mechanism for the principal. 

\begin{restatable}{theorem}{thoptuncor}\label{th:thoptuncor}
	If there exist a prior $\pvec\in\Delta(\Theta)$ and some signaling schemes $\psi_i(\cdot\vert b, \theta)$, for $i\in\mc N$, $b\in B_i$ and $\theta\in\Theta$ that satisfy Equation \eqref{eq:uncorrprob}, then there exists a mechanism $(\muvec, \gammavec, \pivec)\in\U$ that is a solution to optimization problem \eqref{eq:genopt}
\end{restatable}

As a consequence of Theorem \label{eq:thoptuncor}, if Equation \eqref{eq:uncorrprob} is satisfied, then in order to find an optimal mechanism one can restrict the feasibility set of optimization problem $\eqref{eq:genopt}$ to uncorrelated mechanisms, thus significantly reducing the complexity of finding such an optimal mechanism. 

\subsection{Games with Peer-Dependent Signals: the Power of Correlated Mechanisms}

When the signal received by an agent, is influenced by the actions played by the others, we call the game a Peer-Dependent Signals (PDS) game. When considering these games, we do not assume a particular structure on the joint probability $\prob\left(\svec, \theta\vert\bvec\right)$, and allow any possible correlation between signals, states of nature and actions. Like for PIS games, we provide an example that shows how PDS games can be used to model real-world information acquisition scenarios.

\begin{example}[PDS Games]
	\fe{TODO}
\end{example}

Differently than PIS games, when considering PDS games, the adoption of correlated mechanisms can become crucial for the principal in order to be able to decrease the overall payments needed to incentivize action profiles that provide useful information on the state of nature. 

Theorem \ref{th:thoptcor} strengthens the role and the importance of correlation in the mechanism design problems that we investigate. As a consequence of this, when facing an unknown game (as it is the case of the online learning scenario that we study next) it is not possible to establish a priori whether we can restrict to uncorrelated mechanisms and exploit an online learnig algorithm formulation similar to \cite{chen2023learning}.

